Scalable Syntax-Aware Language Models Using Knowledge Distillation

Prior work has shown that, on small amounts of training data, syntactic neural language models learn structurally sensitive generalisations more successfully than sequential language models. However, their computational complexity renders scaling difficult, and it remains an open question whether structural biases are still necessary when sequential models have access to ever larger amounts of training data. To answer this question, we introduce an efficient knowledge distillation (KD) technique that transfers knowledge from a syntactic language model trained on a small corpus to an LSTM language model, hence enabling the LSTM to develop a more structurally sensitive representation of the larger training data it learns from. On targeted syntactic evaluations, we find that, while sequential LSTMs perform much better than previously reported, our proposed technique substantially improves on this baseline, yielding a new state of the art. Our findings and analysis affirm the importance of structural biases, even in models that learn from large amounts of data.

==> Equations.tex <==
Here we outline the knowledge distillation (KD) approach to transfer a hierarchical bias from the teacher RNNG to the student LSTM. Before describing the distillation objective, we begin by casting the standard language modelling objective as finding a set of parameters $\hat{\theta}_{\text{LM}}$ that would minimise the Kullback–Leibler (KL) divergence between the empirical distribution $p^{\mathbf{*}}(\boldsymbol{x})$ and an LSTM learner parameterising $q_{\theta}(\boldsymbol{x})$:
\vspace{-2mm}
\begin{align*}
    &\hat{\theta}_{\text{LM}} = \argmin_{\theta} D_{\mathrm{KL}} \left( p^{\mathbf{*}}(\boldsymbol{x}) \,\,|| \,\, q_{\theta}(\boldsymbol{x}) \right), \\
    &=  \argmin_{\theta} \sum_{\boldsymbol{x} \in \Sigma^{\mathbf{*}}} \left[ p^{\mathbf{*}}(\boldsymbol{x}) \log p^{\mathbf{*}}(\boldsymbol{x})  - p^{\mathbf{*}}(\boldsymbol{x}) \log q_{\theta}(\boldsymbol{x}) \right],
\end{align*}
where $\Sigma$ the set of all word types in the vocabulary, $\Sigma^{\mathbf{*}}$ the space of all possible sentences, $\boldsymbol{x} \in \Sigma^{\boldsymbol{*}}$ denotes a particular sentence with length $|\boldsymbol{x}|$, and $\theta$ the set of LSTM parameters. By removing terms that do not depend on $\theta$, we obtain the familiar cross-entropy objective:
\begin{align}
     \hat{\theta}_{\text{LM}} = \argmin_{\theta} -\sum_{\boldsymbol{x} \in \Sigma^{\mathbf{*}}} p^{\mathbf{*}}(\boldsymbol{x}) \log q_{\theta}(\boldsymbol{x}). \label{eq:objective}
\end{align}

For a dataset of sentences $D = \{\boldsymbol{x}^{(1)}, \ldots, \boldsymbol{x}^{(|D|)} \}$ characterising the empirical distribution $p^{\mathbf{*}}(\boldsymbol{x})=\frac{1}{|D|}$ when $\boldsymbol{x} \in D$, the optimisation objective above becomes:
\vspace{-2mm}
\begin{align*}
    \hat{\theta}_{\text{LM}} &= \argmin_{\theta} - \dfrac{1}{|D|} \sum_{\boldsymbol{x} \in D} \log q_{\theta}(\boldsymbol{x}), \\
    &= \argmin_{\theta} - \dfrac{1}{|D|} \sum_{\boldsymbol{x} \in D} \sum_{j=1}^{|\boldsymbol{x}|} \log q_{\theta}(x_j \mid \boldsymbol{x_{<j}}),
\end{align*}
which reduces to the standard optimisation objective for a left-to-right LSTM LM.

In this work, we aim to transfer the structural bias of a teacher RNNG to a sequential LSTM through KD. We thus substitute the empirical distribution $p^{\mathbf{*}}(\boldsymbol{x})$ in Eq.~\ref{eq:objective} and instead minimise the KL divergence between the pre-trained RNNG's marginal probability $t(\boldsymbol{x}) = \sum_{\boldsymbol{y} \in \mathcal{T}(\boldsymbol{x})} t(\boldsymbol{x}, \boldsymbol{y})$ and the LSTM student $q_{\theta}(\boldsymbol{x})$:
\vspace{-2mm}
\begin{align}
     \hat{\theta}_{\text{KD}} &= \argmin_{\theta} -\sum_{\boldsymbol{x} \in \Sigma^{\mathbf{*}}} t(\boldsymbol{x}) \log q_{\theta}(\boldsymbol{x}), \label{eq:distill_obj} \\
     &= \argmin_{\theta} - \E_{\boldsymbol{x} \sim t(\boldsymbol{x})}  \log q_{\theta}(\boldsymbol{x}).
\end{align}
Since Eq.~\ref{eq:distill_obj} involves an intractable summation over the space of all possible sentences and all possible trees, one alternative is to use Monte Carlo sampling to obtain $K$ sentences $D' = \{\boldsymbol{x}'^{(1)}, \ldots, \boldsymbol{x}'^{(K)}\}$ from $t(\boldsymbol{x})$,\footnote{While an RNNG estimates $t(\boldsymbol{x}, \boldsymbol{y})$, a simple way of sampling surface strings $\boldsymbol{x}$ from the RNNG is to sample pairs of $(\boldsymbol{x}^{(k)}, \boldsymbol{y}^{(k)}) \sim t(\boldsymbol{x}, \boldsymbol{y})$ and ignore all non-terminals $\boldsymbol{y}^{(k)}$.} and train a student LSTM on these sampled sentences as opposed to ground-truth ones:
\vspace{-4mm}
\begin{align}
     \E_{\boldsymbol{x} \sim t(\boldsymbol{x})}  \log q_{\theta}(\boldsymbol{x})
     \approx \dfrac{1}{K} \sum_{\boldsymbol{x}' \in D'} \sum_{j=1}^{|\boldsymbol{x}'|} \log q_{\theta}(x'_j | \boldsymbol{x}'_{<j}). \label{eq:sampling_rnng}
\end{align}
Unfortunately, this procedure suffers from high variance due to the enormity of the sample space. Our preliminary experiments indicate that training the student LSTM on the same number of sampled sentences as the training set size (i.e. $K\approx3,000,000$) from the teacher model results in a much worse validation perplexity than the standard LSTM LM \ask{TODO}. 

We instead minimise the KL divergence between the teacher and student models at the \emph{local word-level} rather than entire sequences. By applying the i.i.d. assumption to the predictions of each word, Eq.~\ref{eq:distill_obj} is approximated as follows:
\vspace{-2mm}
\begin{align*}
    & -\sum_{\boldsymbol{x} \in \Sigma^{\mathbf{*}}} t(\boldsymbol{x}) \log q_{\theta}(\boldsymbol{x}) =  - \E_{\boldsymbol{x} \sim t(\boldsymbol{x})}  \log q_{\theta}(\boldsymbol{x}),\\
    &\approx - \E_{\boldsymbol{x} \sim p^{\mathbf{*}}(\boldsymbol{x})}\,  \sum_{j=1}^{|\boldsymbol{x}|}  D_{\mathrm{KL}} \left( t(w \mid \boldsymbol{x}_{<j}) \,\,|| \,\, q_{\theta}(w \mid \boldsymbol{x}_{<j}) \right),
\end{align*}
where $\boldsymbol{x}$ is sampled from the empirical distribution $p^{\mathbf{*}}(\boldsymbol{x})$, as opposed to the teacher RNNG in Eq.~\ref{eq:sampling_rnng}. Here $t(w \mid \boldsymbol{x}_{<j}})$ and $q_{\theta}(w \mid \boldsymbol{x}_{<j})$ respectively parameterise the (marginal) probability of generating the next-word continuation $w \in \Sigma$, given a conditioning context $\boldsymbol{x}_{<j}$ from the empirical distribution, under the teacher and student models. By expanding the KL term and removing terms that are independent of $\theta$, the word-level KD objective for a dataset $D$ is thus:
\vspace{-2mm}
\begin{align}
  &\hat{\theta}_{\text{KD}} \approx \argmin_{\theta} - \dfrac{1}{|D|} \sum_{\boldsymbol{x} \in D} \ell_{\text{KD}}(\boldsymbol{x}; \theta), \\
  &\ell_{\text{KD}}(\boldsymbol{x}; \theta) =  \sum_{j=1}^{|\boldsymbol{x}|} \sum_{w \in \Sigma} t(w \mid \boldsymbol{x}_{<j}) \log q_{\theta}(w \mid \boldsymbol{x}_{<j}). \label{eq:dist_loss}
\end{align}
In other words, for each word in a training sentence we minimise the cross-entropy between the softmax distributions for the next word of the teacher RNNG and student LSTM. %While this objective has been applied for language modelling by \newcite{furlanello_18}, \lr{be a little more specific about Furlanello so the novelty of your contribution is clear} here we derive the connection between sequence-level and word-level KD as an additional contribution. 

%\ignore{\footnote{For instance, a na\"ive way of computing $t(w \mid \boldsymbol{x}_{<j})$ is to run the word-synchronised beam search procedure to infer the single most likely \emph{partial} tree for $\mathbf{x_{<j}}$, denoted as $\mathbf{\hat{y}_{<j}}$. Using $(\mathbf{x_{<j}}, \mathbf{\hat{y}_{<j}})$ as the conditioning context, we can assume $t(w | \mathbf{x_{<j}}) \approx t(w | \mathbf{x_{<j}}, \mathbf{\hat{y}_{<j}})$ and then perform Monte Carlo sampling (ignoring non-terminals) to compute an estimate of $t(w | \mathbf{x_{<j}}, \mathbf{\hat{y}_{<j}})$. This procedure, however, is too costly to run on all $\sim$ 3M training sentences.\ask{Need help}}}

==> Full_table.tex <==
\begin{table*}[t]
      \centering
      \resizebox{\textwidth}{!}{%
       \begin{tabular}{l|r|r||r|r|r||r||r}
       & \multicolumn{2}{c||}{\textbf{Small Training Set}} & \multicolumn{3}{c||}{\textbf{Full Training Set}} \\ \hline
		& \textbf{S-DSA-LSTM}$^{\dagger}$ &  \textbf{RNNG}$^{\dagger}$ & \textbf{Full LSTM} & \textbf{BA-LSTM} & \textbf{DSA-LSTM} &\textbf{BERT} & \textbf{Humans}  \\
		\hline\hline
		\newcite{gulordava_18} \textbf{test ppl.} & 93.95 ($\pm$0.18)  & 92.30 ($\pm$0.27) & \textbf{53.73} ($\pm$0.16)  &  54.64 ($\pm$0.25) &  56.74 ($\pm$0.26) & N/A & N/A \\ \hline \hline
	    \multicolumn{8}{c}{SUBJECT-VERB AGREEMENT}  \\ \hline
		Simple & 0.96 ($\pm$0.03)  & 0.83 & \textbf{1.00} ($\pm$0.00)  & \textbf{1.00} ($\pm$0.00)  & \textbf{1.00} ($\pm$0.00) & 1.00 & 0.96 \\ 
        In a sentential complement & 0.98 ($\pm$0.02)  & 0.94 & 0.97 ($\pm$0.02) & \textbf{0.98} ($\pm$0.02) & \textbf{0.98} ($\pm$0.02) & 0.83 & 0.93 \\ 
        Short VP coordination &  0.88 ($\pm$0.04) & 0.79 & 0.96 ($\pm$0.02) & 0.95 ($\pm$0.02)  & \textbf{0.99} ($\pm$0.02)   & 0.89 & 0.94 \\ 
        Long VP coordination & 0.74 ($\pm$0.03) & 0.65 & \textbf{0.82} ($\pm$0.05) & 0.80 ($\pm$0.04)  & 0.80 ($\pm$0.02)   & 0.98 & 0.82 \\ 
        Across a prepositional phrase & 0.88 ($\pm$0.02)   & 0.85 & 0.89 ($\pm$0.02)  & 0.89 ($\pm$0.03)  & \textbf{0.91} ($\pm$0.03)  & 0.85 & 0.85 \\ 
        Across a subject relative clause & 0.87 ($\pm$0.02) & 0.71 & 0.87 ($\pm$0.02)  & 0.87 ($\pm$0.01)  & \textbf{0.90} ($\pm$0.02) & 0.84 & 0.88 \\
        Across an object relative clause & 0.69 ($\pm$0.06) & 0.90 & 0.77 ($\pm$0.11)  &  0.81 ($\pm$0.05) & \textbf{0.84} ($\pm$0.03) & 0.89 & 0.85 \\
        Across an object relative clause (no \emph{that}) & 0.61 ($\pm$0.05) & 0.90 & 0.70 ($\pm$0.05)  & 0.74 ($\pm$0.03)  & \textbf{0.77} ($\pm$0.02) & 0.86 & 0.82 \\
        In an object relative clause & 0.87 ($\pm$0.05) & 0.81 & 0.90 ($\pm$0.03)  & 0.91 ($\pm$0.03)  & \textbf{0.92} ($\pm$0.04) & 0.95 & 0.78 \\
        In an object relative clause (no \emph{that}) & 0.88 ($\pm$0.03) & 0.76 & 0.86 ($\pm$0.05)  & 0.83 ($\pm$0.02)  & \textbf{0.92} ($\pm$0.02) & 0.79 & 0.79 \\ \hline
         \textbf{Average of subject-verb agreement} & 0.84 ($\pm$0.02)  & 0.81 & 0.87 ($\pm$0.02) & 0.88 ($\pm$0.01)  & \textbf{0.90} ($\pm$0.01) & 0.89 & 0.86 \\ \hline \hline
        \multicolumn{8}{c}{REFLEXIVE ANAPHORA}  \\ \hline
        Simple & 0.90 ($\pm$0.01) & 0.90 & 0.91 ($\pm$0.01)  & \textbf{0.92} ($\pm$0.03)  & 0.91 ($\pm$0.04) & 0.94 & 0.96\\ 
       In a sentential complement & 0.78 ($\pm$0.01)  & 0.91 & 0.81 ($\pm$0.02)  & 0.81 ($\pm$0.02)  & \textbf{0.82} ($\pm$0.03) & 0.89 & 0.91  \\ 
       Across a relative clause & 0.67 ($\pm$0.03)  & 0.94 & 0.64 ($\pm$0.02)  & 0.64 ($\pm$0.02)  & \textbf{0.67} ($\pm$0.03) & 0.80 & 0.87  \\ \hline
        \textbf{Average of reflexive anaphora} & 0.78 ($\pm$0.01)  & \textbf{0.92} & 0.79 ($\pm$0.01)   & 0.79 ($\pm$0.02)  & \textbf{0.80} ($\pm$0.03) & 0.88 & 0.91 \\ \hline \hline
       \multicolumn{8}{c}{NEGATIVE POLARITY ITEMS}  \\ \hline
       Simple & 0.84 ($\pm$0.05) & 0.61 & 0.96 ($\pm$0.04)  & \textbf{0.98} ($\pm$0.02)  & 0.94 ($\pm$0.04) & N/A & 0.98 \\ 
       Across a relative clause & 0.73 ($\pm$0.07)  & 0.96 & 0.75 ($\pm$0.12) & 0.70 ($\pm$0.10)  & \textbf{0.91} ($\pm$0.07) & N/A &  0.81  \\ \hline
        \textbf{Average of negative polarity items} & 0.79 ($\pm$0.05)  & 0.79 & 0.86 ($\pm$0.06)  & 0.84 ($\pm$0.05)  & \textbf{0.92} ($\pm$0.05) & N/A & 0.90 \\ \hline \hline
       \textbf{Average of all constructions} & 0.82 ($\pm$0.02)  & 0.83 & 0.85 ($\pm$0.02)  & 0.86 ($\pm$0.01)  & \textbf{0.89} ($\pm$0.01) & N/A &  0.88  
		\end{tabular}}
		\caption{Comparison of the \textbf{DSA-LSTM} with four baselines. \textbf{S-DSA-LSTM} indicates the DSA-LSTM trained on the smaller RNNG training set, while \textbf{BA-LSTM} is the born-again baseline where the teacher is an LSTM trained on the full training set. We also compare with the syntactic generalisation of \textbf{BERT} Base\footnote{Here we choose the BERT Base as opposed to the BERT Large model, since the former generally performs better on targeted syntactic evaluation \cite{goldberg_2019}.} \cite{devlin_2018,goldberg_2019}, which is not strictly comparable since it operates non-incrementally and is trained on 30 times as much data. $^{\dagger}$ indicates models trained on the smaller 20\% training set (\S3). Results in bold denote the best among those trained with the same amounts of data.}
        \label{tab:dsa-lstm}
\end{table*}
